Accelerated Convergence of Stochastic Heavy Ball Method under Anisotropic Gradient Noise

Heavy-ball momentum with decaying learning rates is widely used with SGD for optimizing deep learning models. In contrast to its empirical popularity, the understanding of its theoretical property is still quite limited, especially under the standard anisotropic gradient noise condition for quadratic regression problems. Although it is widely conjectured that heavy-ball momentum method can provide accelerated convergence and should work well in large batch settings, there is no rigorous theoretical analysis. In this paper, we fill this theoretical gap by establishing a non-asymptotic convergence bound for stochastic heavy-ball methods with step decay scheduler on quadratic objectives, under the anisotropic gradient noise condition. As a direct implication, we show that heavy-ball momentum can provide $\tilde{\mathcal{O}}(\sqrt{\kappa})$ accelerated convergence of the bias term of SGD while still achieving near-optimal convergence rate with respect to the stochastic variance term. The combined effect implies an overall convergence rate within log factors from the statistical minimax rate. This means SGD with heavy-ball momentum is useful in the large-batch settings such as distributed machine learning or federated learning, where a smaller number of iterations can significantly reduce the number of communication rounds, leading to acceleration in practice.

==> assumptions_discussion.tex <==
\newcommand{\bW}{\mathbf{W}}
\section{Discussion of the Assumptions}\label{appendix:assumption_discussion}
In this section, we discuss how to adapt our proof to the standard least-square regression setting. 
We work on the least-square problem
\begin{align*}
    \min_{\bw\in\mathbb{R}^d} f(\bw), \text{ where } f(\bw) \overset{\text{def}}{=} \frac{1}{2}\mathbb{E}_{(\xb,y)\thicksim\mathcal{D}}\left[(y-\dotprod{\xb,\bw})^2 \right].
\end{align*}
And its stochastic gradient oracle is
\begin{align*}
    \widehat \nabla f(\bw) = -(y-\dotprod{\xb,\bw}) \cdot \xb.
\end{align*}
For simplicity, we use $\mathbb{E}$ to denote $\mathbb{E}_{(\xb,y)\thicksim\mathcal{D}}$ in the rest of this section. We further denote that
\begin{align*}
    \mathbb{E}\left[ \xb\xb^\top\right]=\bH
\end{align*}
and assume $y=\dotprod{\xb,\bw_*}+\epsilon$, where $\bw_*$ is the global optimum. 
\begin{assumption}[Covariance]\label{ass:covariance}
    There exists constant $\Tilde{\sigma}^2$, such that
    \begin{align*}
        \mathbb{E}\left[\epsilon^2\cdot \xb\xb^\top\right] \preceq \Tilde{\sigma}^2\bH.
    \end{align*}
\end{assumption}
\begin{assumption}[Finite fourth momentum]\label{ass:fourth_moment}
    There exists constant $R^2$, such that
    \begin{align*}
        \mathbb{E}\left[\norm{\xb}^2\cdot \xb\xb^\top\right] \preceq R^2\bH.
    \end{align*}
\end{assumption}
\begin{assumption}[Statistical condition number]\label{ass:statistical_condition_number}
There exists constant $\Tilde{\kappa}$, such that
    \begin{align*}
        \mathbb{E}\left[\xb^\top\bH^{-1}\xb\cdot \xb\xb^\top\right] \preceq \Tilde{\kappa}\bH.
    \end{align*}
\end{assumption}
Here Assumption~\ref{ass:covariance} and \ref{ass:fourth_moment} are standard assumptions of least-square regression~(\citet{bach2013non,jain2016parallelizing,ge2019step}).  Assumption~\ref{ass:statistical_condition_number} is used in \citet{jain2018accelerating} and $\Tilde{\kappa}$ is denoted as the statistical condition number. As $\mathbb{E}\left[\xb^\top\bH^{-1}\xb\cdot \xb\xb^\top\right]\preceq\frac{1}{\mu}\mathbb{E}\left[\xb^\top\xb\cdot \xb\xb^\top\right]\preceq(R^2/\mu)\bH$, it holds that $\Tilde{\kappa}\le R^2/\mu$.
And from the first optimality condition, it holds that
    \begin{align*}
        \nabla f(\bw_*)=\mathbb{E}\left[\epsilon \xb\right] = 0.
    \end{align*}
% \begin{proposition}[First order optimality condition]
%     % It holds that
%     \begin{align*}
%         \nabla f(\bw_*)=\mathbb{E}\left[\epsilon \xb\right] = 0
%     \end{align*}
% \end{proposition}
% It is worth pointing out that in the standard assumptions, they don't assume $\xb$ and $\epsilon$ are independent. In fact the case that $\epsilon$ is independent from $\xb$ is called the homoscedastic (additive noise/well specified) case. In this case, assumption \ref{ass:covariance} can be changed to use equality. The standard papers~(\citet{bach2013non,ge2019step,jain2016parallelizing}) don't assume this. 
In this paper, we additionally assume that $\bw$ is in a compact set, which is formally stated in Assumption~\ref{ass:compact_set}.
\begin{assumption}[Compact set]\label{ass:compact_set}
    For every $t=\{0,1,...\}$, $\bw_t\in\Lambda(\alpha)$, where
    \begin{align*}
        \Lambda=\left\{\bw|(\bw-\bw_*)\bH(\bw-\bw_*)\preceq\alpha^2\right\}.
    \end{align*}
\end{assumption}
\textcolor{blue}{This assumption is mild as it is common in practical neural network training. Please refer to TODO for more details.} 
\begin{lemma}[Transformation to least-square problem]\label{lem:transform_least_square}
    Under Assumption~\ref{ass:covariance}, \ref{ass:fourth_moment}, \ref{ass:statistical_condition_number} and \ref{ass:compact_set}, it holds that
    \begin{align*}
        \sigma^2 \le 2\left[ \alpha^2(\Tilde{\kappa}-1)+\Tilde{\sigma}^2 \right]
    \end{align*}
    and the result under Assumption~\ref{ass:independent_noise}, \ref{ass:unbiased_noise} and \ref{ass:anisotropic_noise} can be transferred to result under Assumption~\ref{ass:covariance}, \ref{ass:fourth_moment}, \ref{ass:statistical_condition_number} and \ref{ass:compact_set} by replacing $\sigma^2$ with $2\left[ \alpha^2(\Tilde{\kappa}-1)+\Tilde{\sigma}^2 \right]$.
\end{lemma}
\begin{proof}
The gradient noise $\bn_t$ is
\begin{align*}
    \bn_t &= \nabla f(\bw_t) - \widehat \nabla f(\bw_t) 
    = \bH\bw_t - b + (y_t-\dotprod{\xb_t,\bw_t}) \cdot \xb_t \\
    &= \bH(\bw_t-\bw_*) + (\epsilon_t+\dotprod{\xb_t,\bw_*-\bw_t}) \cdot \xb_t \\
    &= (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)
    +\epsilon_t\xb_t.
\end{align*}
Thus Assumption~\ref{ass:independent_noise} and \ref{ass:unbiased_noise} hold as $\EE[\epsilon\xb]=0$.
And it holds that
\begin{align*}
    \bn_t\bn_t^\top 
    =& \left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)
    -\epsilon_t\xb_t\right] \left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)
    -\epsilon_t\xb_t\right]^\top \\
    \preceq& 2(\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)+ 2\epsilon_t^2 \xb_t\xb_t^\top,
\end{align*}
where the inequality uses the fact that $(\xb+y)(x+y)^\top\preceq 2(xx^\top+yy^\top)$. Thus we have
% \begin{align*}
%     \mathbb{E}\left[ \bn_t\bn_t^\top\right]\preceq&
%     2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)+ \epsilon_t^2 \xb_t\xb_t^\top\right] \\
%     \preceq&
%     2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)\right]+2\Tilde{\sigma}^2 \bH \\
%     =&
%     2\mathbb{E}\left[ \xb_t^\top\bW_t\xb_t\xb_t\xb_t^\top\right]-2\bH\bW_t\bH+2\Tilde{\sigma}^2 \bH
% \end{align*}
where $\bW_t=(\bw_t-\bw_*)(\bw_t-\bw_*)^\top$. With Assumption~\ref{ass:compact_set}, it holds that $\bW_t \preceq \alpha^2 \bH^{-1}$. And thus
\begin{align*}
    \mathbb{E}\left[\bn_t\bn_t^\top\right] \preceq & 2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)\right]+2\Tilde{\sigma}^2\bH \\
        \preceq&
        2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\alpha^2\bH^{-1})(\bH-\xb_t\xb_t^\top)\right]+2\Tilde{\sigma}^2\bH \\ 
        =& 2\alpha^2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)\bH^{-1}(\bH-\xb_t\xb_t^\top)\right]+2\Tilde{\sigma}^2\bH \\
        =&
        2\alpha^2\mathbb{E}\left[ \xb^\top\bH^{-1}\xb\xb\xb^\top-\bH\right]+2\Tilde{\sigma}^2\bH \preceq 2\alpha^2\left( \Tilde{\kappa}\bH-\bH\right) +2\Tilde{\sigma}^2\bH.
\end{align*}
Therefore, Assumption \ref{ass:anisotropic_noise} hold with $\sigma^2$ replaced by $2\left[ \alpha^2(\Tilde{\kappa}-1)+\Tilde{\sigma}^2 \right]$. And thus with Assumption~\ref{ass:independent_noise}, \ref{ass:unbiased_noise} and \ref{ass:anisotropic_noise} hold, the result can be transferred to the least-square setting.
\end{proof}

Therefore, with Lemma~\ref{lem:transform_least_square}, we can formally state our result in least-square setting.

\begin{corollary}[Result in least-square setting]\label{cor:least_square}
    Under Assumption~\ref{ass:covariance}, \ref{ass:fourth_moment}, \ref{ass:statistical_condition_number} and \ref{ass:compact_set} and the requirements of learning rate schedule and momentum in Theorem~\ref{thm:main}, the output of Algorithm~\ref{alg:multistage_sgdm} satisfies 
    \begin{align*}
        \EE\left[f(\bw_T)-f(\bw_*)\right] \le& \mathbb{E}\left[ f(\bw_0)-f(\bw_*) \right]\cdot \exp\left(-\tilde{\Omega}\left(\frac{T}{\sqrt{\kappa}}\right)\right)
        +
        \tilde{\cO}\left( \frac{d\Tilde{\sigma}^2}{MT}\right) \\
        &+\tilde{\cO}\left( \frac{d\alpha^2\Tilde{\kappa}}{MT}\right),
    \end{align*}
    where $\Tilde{\cO}(\cdot)$ and $\Tilde{\Omega}(\cdot)$ are used to hide the log factors.
\end{corollary}

% \textcolor{blue}{Discussion for using how many iterations?}

% \subsection{Experiemnt Details}
% I set $N=10101$ samples and let the samples to be
% \begin{align*}
%     x =& \begin{bmatrix}
%         1 \\ 0 \\ 0
%     \end{bmatrix}, \qquad\text{with probability}\quad \frac{1}{10101} \\
%     x =& \begin{bmatrix}
%         0 \\ 1 \\ 0
%     \end{bmatrix}, \qquad\text{with probability}\quad \frac{100}{10101} \\
%     x =& \begin{bmatrix}
%         0 \\ 0 \\ 1
%     \end{bmatrix}, \qquad\text{with probability}\quad \frac{10000}{10101} \\
% \end{align*}
% And thus we have
% \begin{align*}
%     \bH = \mathbb{E}\left[ xx^\top\right]=& \frac{1}{10101} \begin{bmatrix}
%         1 & & \\ & 100 & \\ & & 10000
%     \end{bmatrix} \\ 
%     \mathbb{E} \left[x^\top xxx^\top\right]=&\frac{1}{10101}\begin{bmatrix}
%         1 & & \\ & 100 & \\ & & 10000
%     \end{bmatrix} \\
%     \mathbb{E} \left[x^\top\bH^{-1} xxx^\top\right]=&\begin{bmatrix}
%         1 & & \\ & 1 & \\ & & 1
%     \end{bmatrix}
% \end{align*}
% Thus we have $R^2=1,\mu\approx 1e-4$, and thus $\kappa\approx10^4$, $\Tilde{\kappa}\approx10^4$.

% We set $\alpha^2= 1/3$ and with noise $\epsilon\thicksim N(0,\Tilde{\sigma}^2=0.01)$, we have noise $\sigma^2$ satisfying
% \begin{align*}
%     \mathbb{E}\left[\bn\bn^\top\right] \preceq \sigma^2 \bH
% \end{align*}
% and we find that $\sigma^2\approx 1$. 
% We have some key observations:
% \begin{itemize}
%     \item It may be better to use ball compact set $(\wb_0-\wb_*)^\top(\wb_0-\wb_*)\le \alpha^2$. In this case $\sigma^2\approx \alpha^2R^2$ is almost tight. But this may depend on the problem.
%     \item $\sigma^2$ and $\Tilde{\sigma}^2$ is different, which supports our theoretical analysis.
% \end{itemize}

% Let's discuss how to address the covariance $\sigma^2$ now.
% The gradient noise $\bn_t$ can be represented as
% \begin{align*}
%     \bn_t = \nabla f(\bw_t) - \widehat \nabla f(\bw_t) = (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)
%     -\epsilon_t\xb_t
% \end{align*}
% and we have that
% \begin{align*}
%     \bn_t\bn_t^\top 
%     % =& (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top) - \epsilon_t\xb_t(\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*) \\
%     % &- \epsilon_t(\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)\xb_t^\top + \epsilon_t^2 \xb_t\xb_t^\top
%     =& \left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)
%     -\epsilon_t\xb_t\right] \left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)
%     -\epsilon_t\xb_t\right]^\top \\
%     \preceq& 2(\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)+ 2\epsilon_t^2 \xb_t\xb_t^\top,
% \end{align*}
% where the inequality uses the fact that $(\xb+y)(x+y)^\top\preceq 2(xx^\top+yy^\top)$. Thus we have
% \begin{align*}
%     \mathbb{E}\left[ \bn_t\bn_t^\top\right]\preceq&
%     2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)+ \epsilon_t^2 \xb_t\xb_t^\top\right] \\
%     \preceq&
%     2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)\right]+2\Tilde{\sigma}^2 \bH \\
%     =&
%     2\mathbb{E}\left[ \xb_t^\top\bW_t\xb_t\xb_t\xb_t^\top\right]-2\bH\bW_t\bH+2\Tilde{\sigma}^2 \bH
% \end{align*}
% where $\bW_t=(\bw_t-\bw_*)(\bw_t-\bw_*)^\top$. If we additionally assume that $\bw_t$ is in a compact set, here we may have two possible cases, one is isotropic and the other one is anisotropic. 
% \begin{assumption}[isotropic compact set]\label{ass:isotropic_compact_set}
%     For every $t=\{0,1,...\}$, 
%     \begin{align*}
%         \norm{\bw_t-\bw_*}^2 \le \alpha^2 \quad\text{or equivalently}\quad (\bw_t-\bw_*)(\bw_t-\bw_*)^\top \preceq \alpha^2\bI.
%     \end{align*}
%     % where
%     % \begin{align*}
%     %     \alpha^2 = \frac{\Tilde{\sigma}^2}{R^2-\mu}.
%     % \end{align*}
% \end{assumption}
% \begin{proposition}
%     With Assumption \ref{ass:fourth_moment}, \ref{ass:covariance} and \ref{ass:isotropic_compact_set}, it holds that
%     \begin{align*}
%         \mathbb{E}\left[ \bn_t\bn_t^\top\right] \preceq 2\left[\alpha^2\left(R^2-\mu\right)+\Tilde{\sigma}^2\right] \bH
%     \end{align*}
% \end{proposition}
% \begin{proof}
%     Using the conditions, we have
%     \begin{align*}
%         &\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)\right] \\
%         \preceq&
%         \mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\alpha^2\bI)(\bH-\xb_t\xb_t^\top)\right] = \alpha^2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bH-\xb_t\xb_t^\top)\right] \\
%         =&
%         \alpha^2\mathbb{E}\left[ \norm{\xb}^2\xb\xb^\top-\bH^2\right] \preceq \alpha^2\left( R^2\bH-\bH^2\right) \\
%         =&
%         \alpha^2 \norm{R^2\bI-\bH}\bH \preceq \alpha^2\left(R^2-\mu\right)\bH,
%     \end{align*}
%     where in the first inequality, we use the property of Loewner order. Substituting we can obtain the result.
% \end{proof}

% Thus in this case, with additional assumption \ref{ass:isotropic_compact_set}, we can use their assumptions and simply replace $\sigma^2$ with $4\Tilde{\sigma}^2$. 

% For anisotropic setting, we need to further use an additional assumption as used in \citet{jain2016parallelizing}.
% \begin{assumption}[anisotropic fourth moment]\label{ass:anisotropic_fourth_moment}
%     It holds that
%     \begin{align*}
%         \mathbb{E}\left[\xb^\top\bH^{-1}\xb \xb\xb^\top \right] \preceq \Tilde{\kappa} \bH,
%     \end{align*}
%     where $\Tilde{\kappa}$ is called the statistical condition number in \citet{jain2016parallelizing}, which is smaller than $R^2/\mu$.
% \end{assumption}
% \begin{assumption}[anisotropic compact set]\label{ass:anisotropic_compact_set}
%     For every $t=\{0,1,...\}$, 
%     \begin{align*}
%         (\bw_t-\bw_*)\bH(\bw_t-\bw_*)\preceq\alpha^2 \quad \text{or equivalently}\quad (\bw_t-\bw_*)(\bw_t-\bw_*)^\top \preceq \alpha^2 \bH^{-1}.
%     \end{align*}
%     % where
%     % \begin{align*}
%     %     \alpha^2 = \frac{\Tilde{\sigma}^2}{\Tilde{\kappa}-1}.
%     % \end{align*}
% \end{assumption}
% \begin{proposition}
%     With Assumption \ref{ass:fourth_moment}, \ref{ass:covariance}, \ref{ass:anisotropic_fourth_moment} and \ref{ass:anisotropic_compact_set}, it holds that
%     \begin{align*}
%         \mathbb{E}\left[ \bn_t\bn_t^\top\right] \preceq 2\left[\alpha^2\left(\Tilde{\kappa}-1\right)+\Tilde{\sigma}^2\right] \bH
%     \end{align*}
% \end{proposition}
% \begin{proof}
%     Using the conditions, it holds that
%     \begin{align*}
%         &\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\bw_t-\bw_*)(\bw_t-\bw_*)^\top(\bH-\xb_t\xb_t^\top)\right] \\
%         \preceq&
%         \mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)(\alpha^2\bH^{-1})(\bH-\xb_t\xb_t^\top)\right] = \alpha^2\mathbb{E}\left[ (\bH-\xb_t\xb_t^\top)\bH^{-1}(\bH-\xb_t\xb_t^\top)\right] \\
%         =&
%         \alpha^2\mathbb{E}\left[ \xb^\top\bH^{-1}\xb\xb\xb^\top-\bH\right] \preceq \alpha^2\left( \Tilde{\kappa}\bH-\bH\right) \\
%         % =&
%         % \frac{\Tilde{\sigma}^2}{\Tilde{\kappa}-1}\left( \Tilde{\kappa}\bH-\bH\right) \preceq \Tilde{\sigma}^2\bH,
%     \end{align*}
%     where in the first inequality, we use the property of Loewner order. Substituting we can obtain the result.
% \end{proof}
% Thus in this case, with additional assumption \ref{ass:anisotropic_compact_set}, we can use their assumptions and simply replace $\sigma^2$ with $4\Tilde{\sigma}^2$. 

% In this case, our weakness may be
% \begin{enumerate}
%     \item Using additional compact set assumption
%     \item When $\Tilde{\sigma}^2\longrightarrow 0$, \citet{ge2019step} and \citet{jain2016parallelizing} obtain an almost sure geometric convergence, while our result still needs $O(1/T)$ (as the feasible compact set is almost surely empty)
% \end{enumerate}
% And our strength may be
% \begin{enumerate}
%     \item Our result doesn't rely on the fourth moment factor $R^2$, which means that our $\kappa$ is smaller than $R^2/\mu$ used in the standard works.
% \end{enumerate}


% % \textcolor{blue}{If we don't use the homoscedastic setting}, how to? \textcolor{red}{Using Cauchy-Schwarz inequality!}

% \subsection{Is It Suitable to Apply This Assumption?}
% Consider a case that $\bw_0=\bw_*$, which means that the initial point of the algorithm is optimal. However, even in this case, it is still hard to enforce $w_t$ to stay in a compact set. The problem is in this case, we only need to analyze the variance term using $\sigma^2$, and as the algorithm always runs first large stepsizes. For the first $t\le\sqrt{\kappa}$ iterations, the stepsize is all the same and according to the theorem for bounding momentum matrix power, the variance error can be bounded by
% \begin{align*}
%     V_t=&\sigma^2\sum_{k=1}^{t}\eta_k^2\sum_{j=1}^d\lambda_j^2 \norm{\Tb_{1,j}^{k}}^2 \\
%     \le&
%     \sigma^2\sum_{k=1}^{t}\sum_{j=1}^d(\eta'_1)^2\lambda_j^2
%     \left(8k\cdot\rho(\Tb_{1,j})^k \right)^2 \\
%     \approx&
%     \sigma^2\sum_{k=1}^{t}\sum_{j=1}^d\text{ const }\cdot
%     k^2\cdot\rho\left(1-\frac{1}{\sqrt{\kappa}}\right)^{2k} \\ 
%     \approx&
%     d\sigma^2 \cdot \kappa.
% \end{align*}
% Thus $\alpha^2\geq d\sigma^2 \cdot \kappa$
% And substituting to our desired bound that
% \begin{align*}
%     \sigma^2 \geq 2\left[\alpha^2\left(\Tilde{\kappa}-1\right)+\Tilde{\sigma}^2\right] \geq d\sigma^2
% \end{align*}
% we can find that this is not possible as $V_t>\alpha^2$ which means that $\bw_t$ runs out of the compact set. 
% I think this problem implies that the feasible compact set is always smaller than the possible output of iterations, or further that our algorithm may not guarantee convergence in this setting of linear regression. I notice that even SGD~\citet{ge2019step} can not be bounded using this method.

% Thus we possibly we may have only one choice to modify our result to the setting, that is to modify the method in \citet{ge2019step}, where a universal bound for variance is provided. However, we cannot obtain a universal bound for variance as variance is not 

% Consider that we fix $\alpha^2$ as the radius of the compact set. This $\alpha^2$ can be arbitrarily large. Then from our analysis, the gradient noise satisfies that
% \begin{align*}
%     \sigma^2 \geq 2\left[ \alpha^2(\Tilde{\kappa}-1)+\Tilde{\sigma}^2\right] \gtrsim \alpha^2
% \end{align*}
% and also
% \begin{align*}
%     \mathbb{E}\left[\max_{t}\{f(\bw_t)-f(\bw_*) \}\right]
%     \geq& \max_{t}\mathbb{E}\left[\{f(\bw_t)-f(\bw_*) \}\right]
%     \geq V_t \gtrsim d\sigma^2\cdot\kappa \\
%     \geq& d \kappa\cdot \alpha^2
% \end{align*}
% Thus we notice that no matter how large we set the radius of the compact set, the point with the largest error that appears in the iteration will escape the compact set as variance relies on the radius.


% \subsection{Another Possible Way to Claim Linear Regression}
% We can also state that when our analysis can be applied to some kinds of linear regression problem, like stated in \citet{dieuleveut2017harder}, a case where the distribution of $\xb$ is known so that the population covariance matrix is
% computable, but the distribution of the outputs $y$ remains unknown. To claim this, we can just use a section in appendix to give a remark on its application to linear regression.

==> innovation_of_the_proof.tex <==
Technically, the major obstacle is the matrix. the proof is highly dependent on our novel theoretical techniques for analyzing the key properties of the involved $2\times 2$ update matrices. \textcolor{blue}{I think we have to move the lemmas here to talk about the proof as we have to show the $2\times 2$ matrices for better illustration.}
We find that all the elements preserved 
even after adding 
so this property still hold as we combines
which allows us to finding much simple upper bound

==> new_proof_former_version.tex <==
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Jb}{\mathbf{J}}
\renewcommand{\Sb}{\mathbf{S}}
\newcommand{\wb}{\mathbf{w}}
\renewcommand{\cO}[1]{\mathcal{O}\left({#1}\right)}
\newcommand{\Norm}[1]{\left\| #1 \right\|}
\newcommand{\Abs}[1]{\left| #1 \right|}
\newcommand{\skuo}[1]{\left({#1}\right)}


%\newtheorem{lemma}{Lemma}


\setlength{\parindent}{0em}

\subsection{Key Properties of $\norm{\bT_{t,j}}$: $\norm{\bT_{t,j}^k} \Rightarrow \rho(\bT_{t,j})^k$}
\label{appendix:key_property_of_T_tj}

\begin{lemma}[Bounding $\Norm{\Tb_{t,j}^k}_F$ with $\rho(\Tb_{t,j})^k$]\label{lem:1}
    For momentum matrix $\Tb_{t,j}$ that
    \begin{align*}
    \Tb_{t,j}= \left[\begin{matrix}1+\beta-\eta_t\lambda_j&-\beta\\1&0\end{matrix}\right],
    \end{align*}
   and the eigenvalues of $\Tb_{t,j}$ are real, which means that $(1+\beta-\eta_t\lambda_j)^2-4\beta\geq0$. For all positive integer $k$, it holds that 
   \begin{align*}
       \Norm{\Tb_{t,j}^k}_F \le \min\left(8k,\frac{8}{\sqrt{\Abs{(1+\beta-\eta_t\lambda_j)^2-4\beta}}}\right)\rho(\Tb_{t,j})^k.
   \end{align*}
\end{lemma}
\begin{proof}

We can directly analyze the product by Jordan decomposition that there exists $\Pb\in\mathbb{C}^{2\times 2}$ such that
\begin{align*}
    \Tb_{t,j}=\Pb\Jb\Pb^{-1}
\end{align*}
where $\Jb$ can have the following two cases 
\begin{align*}
    \Jb=\left[ \begin{matrix}
        \gamma_1 & 0 \\ 0 & \gamma_2
    \end{matrix}\right] \text{ or }
    \Jb=\left[ \begin{matrix}
        \gamma_1 & 1 \\ 0 & \gamma_2
    \end{matrix}\right]
\end{align*}
depending on whether $\Tb_{t,j}$ is diagnolizable. Here $\gamma_1, \gamma_2$ are the eigenvalues of $\Tb_{t,j}$ and we assume without genarality that $\gamma_1\geq \gamma_2$ if $\gamma_1,\gamma_2\in\mathbb{R}$. And when $\gamma_1,\gamma_2\notin\mathbb{R}$, it holds that $\gamma_1$ and $\gamma_2$ are conjugate thus $\Abs{\gamma_1}=\Abs{\gamma_2}$. Therefore $\gamma_1$ is the spectral radius of $\Tb_{t,j}$, i.e. $\rho(\Tb_{t,j})=\gamma_1$. Then we discuss case by case.

\textbf{i) If $\gamma_1\neq \gamma_2$:} 
In this case one can verify that
\begin{align*}
    \Pb
    =
    \begin{bmatrix}
      \gamma_1 & \gamma_2 \\
      1 & 1
    \end{bmatrix},
    \quad
    \Jb
    =
    \begin{bmatrix}
      \gamma_1 & 0 \\
      0 & \gamma_2
    \end{bmatrix},
    \quad
    \Pb^{-1}
    =
    \frac{1}{\gamma_1 - \gamma_2}
    \begin{bmatrix}
      1 & -\gamma_2 \\
      -1 & \gamma_1
      \end{bmatrix}
\end{align*}
where $\gamma_1,\gamma_2$ are eigenvalues of $\Tb_{t,j}$.
And since the characteristic polynomial of $\Tb_{t,j}$
\begin{align*}
    \det\left(\Tb_{t,j} - \gamma \mathbf{I}\right)
    {=}
    \begin{vmatrix}
      1 + \beta - \eta_t \lambda_j - \gamma & -\beta \\
      1 & -\gamma
    \end{vmatrix}
    =
    \gamma^2
    - \left(1 + \beta - \eta_t \lambda_j\right) \gamma
    + \beta
    =
    0
\end{align*}
entails $\gamma_1 + \gamma_2 = 1 + \beta - \eta_t \lambda_j, \gamma_1 \gamma_2 = \beta$. Thus in this case, we have
\begin{align*}
    \Tb_{t,j}^k &= \Pb\Jb^k\Pb^{-1} = \begin{bmatrix}
      \gamma_1 & \gamma_2 \\
      1 & 1
    \end{bmatrix}
    \cdot
    \begin{bmatrix}
      \gamma_1^k & 0 \\
      0 & \gamma_2^k
    \end{bmatrix}
    \cdot
    \frac{1}{\gamma_1 - \gamma_2}
    \begin{bmatrix}
      1 & -\gamma_2 \\
      -1 & \gamma_1
      \end{bmatrix} \\
      &= \begin{bmatrix}
          \frac{\gamma_1^{k+1}-\gamma_2^{k+1}}{\gamma_1-\gamma_2} & -\beta\frac{\gamma_1^{k}-\gamma_2^{k}}{\gamma_1-\gamma_2} \\ \frac{\gamma_1^{k}-\gamma_2^{k}}{\gamma_1-\gamma_2} &
          -\beta\frac{\gamma_1^{k-1}-\gamma_2^{k-1}}{\gamma_1-\gamma_2}
      \end{bmatrix}. 
\end{align*}
It holds that
\begin{equation*}
\begin{aligned}
    \Norm{\Tb_{t,j}}_F =& \frac{1}{\Abs{\gamma_1-\gamma_2}} \Norm{\begin{bmatrix}
        \gamma_1^{k+1}-\gamma_2^{k+1} & 
        -\beta\left(\gamma_1^{k}-\gamma_2^{k}\right) \\
        \gamma_1^{k}-\gamma_2^{k} &
        -\beta\left(\gamma_1^{k-1}-\gamma_2^{k-1}\right)
    \end{bmatrix}}_F \\
    \le&
    \frac{1}{\Abs{\gamma_1-\gamma_2}}
    \Norm{\begin{bmatrix}
        2\rho(\Tb_{t,j})^{k+1} & 
        -2\beta\rho(\Tb_{t,j})^{k} \\
        2\rho(\Tb_{t,j})^{k} &
        -2\beta\rho(\Tb_{t,j})^{k-1}
    \end{bmatrix}}_F \\
    \le&
    \frac{1}{\Abs{\gamma_1-\gamma_2}}
    \Norm{\begin{bmatrix}
        2\rho(\Tb_{t,j})^{k} & 
        -2\beta\rho(\Tb_{t,j})^{k} \\
        2\rho(\Tb_{t,j})^{k} &
        -4\beta\rho(\Tb_{t,j})^{k}
    \end{bmatrix}}_F 
    \le
    \frac{2\rho(\Tb_{t,j})^{k}}{\Abs{\gamma_1-\gamma_2}}
    \Norm{\begin{bmatrix}
        1 & 
        -\beta \\
        1 &
        -2\beta
    \end{bmatrix}}_F \\
    \le&
    \frac{8\rho(\Tb_{t,j})^{k}}{\Abs{\gamma_1-\gamma_2}}
    =
    \frac{8}{\sqrt{\Abs{(1+\beta-\eta_t\lambda_j)^2-4\beta}}}\rho(\Tb_{t,j})^{k},
\end{aligned}   
\end{equation*}
where the first inequality holds as $\Abs{\gamma_1}=\Abs{\gamma_2}=\rho(\Tb_{t,j})$ and the third inequality holds as $\rho(\Tb_{t,j})\in(1/2,1)$. From another point, it holds that for all $k$,
\begin{equation*}
\begin{aligned}
    \Abs{\frac{\gamma_1^{k}-\gamma_2^{k}}{\gamma_1-\gamma_2}}=\Abs{\sum_{j=0}^{k-1}\gamma_1^j\gamma_2^{k-1-j}} \le
    \sum_{j=0}^{k-1} \Abs{\gamma_1^{j}\gamma_2^{k-1-j} }=\sum_{j=0}^{k-1}\rho(\Tb_{t,j})^{k-1}=k\rho(\Tb_{t,j})^{k-1}.
\end{aligned}
\end{equation*}
Substituting we have
\begin{equation*}
\begin{aligned}
    \Norm{\Tb_{t,j}}_F =& 
    \Norm{\begin{bmatrix}
          \frac{\gamma_1^{k+1}-\gamma_2^{k+1}}{\gamma_1-\gamma_2} & -\beta\frac{\gamma_1^{k}-\gamma_2^{k}}{\gamma_1-\gamma_2} \\ \frac{\gamma_1^{k}-\gamma_2^{k}}{\gamma_1-\gamma_2} &
          -\beta\frac{\gamma_1^{k-1}-\gamma_2^{k-1}}{\gamma_1-\gamma_2}
      \end{bmatrix}}_F \\
      \le&
      \Norm{\begin{bmatrix}
          (k+1)\rho(\Tb_{t,j})^{k} & -\beta k\rho(\Tb_{t,j})^{k-1} \\ k\rho(\Tb_{t,j})^{k-1} &
          -\beta(k-1)\rho(\Tb_{t,j})^{k-2}
      \end{bmatrix}}_F \\
      \le&
      \Norm{\begin{bmatrix}
          2k\rho(\Tb_{t,j})^{k} & -2 k\rho(\Tb_{t,j})^{k} \\ 2k\rho(\Tb_{t,j})^{k} &
          -4k\rho(\Tb_{t,j})^{k}
      \end{bmatrix}}_F 
      \le 8k\rho(\Tb_{t,j})^k.
\end{aligned}
\end{equation*}
Thus we prove the lemma when $\gamma_1\neq \gamma_2$.

\textbf{ii) If $\gamma_1=\gamma_2=\gamma$:} In this case, $\Tb_{t,j}$ can not be diagonalized, which means that
\begin{align*}
    \Tb_{t,j} = \begin{bmatrix}
        \gamma & 1 \\ 0 & \gamma
    \end{bmatrix}
\end{align*}
one can verify that
\begin{align*}
    \Pb
    =
    \begin{bmatrix}
      \gamma & 1 \\
      1 & 0
    \end{bmatrix},
    \quad
    \Jb^k
    =
    \begin{bmatrix}
      \gamma^k & k\gamma^{k-1} \\
      0 & \gamma^k
    \end{bmatrix},
    \quad
    \Pb^{-1}
    =
    \begin{bmatrix}
      0 & 1 \\
      1 & -\gamma
    \end{bmatrix}
\end{align*}
where $\gamma_1=\gamma_2=\gamma\in\mathbb{R}$. In this case, it holds that
\begin{align*}
    \Tb_{t,j}^{k}=\Pb\Jb^{k}\Pb^{-1} &=
    \begin{bmatrix}
      \gamma & 1 \\
      1 & 0
    \end{bmatrix}
    \cdot
    \begin{bmatrix}
      \gamma^k & k\gamma^{k-1} \\
      0 & \gamma^k
    \end{bmatrix}
    \cdot
    \begin{bmatrix}
      0 & 1 \\
      1 & -\gamma
    \end{bmatrix} \\
    &=
    \begin{bmatrix}
        (k+1)\gamma^k & -k\gamma^{k+1} \\
        k\gamma^{k-1} & -(k-1)\gamma^{k}
    \end{bmatrix}
\end{align*}
Then it holds that
\begin{align*}
    \Norm{\Tb_{t,j}^k}_F =& \Norm{\begin{bmatrix}
        (k+1)\gamma^k & -k\gamma^{k+1} \\
        k\gamma^{k-1} & -(k-1)\gamma^{k}
    \end{bmatrix}}_F
    \le
    \Norm{\begin{bmatrix}
        2k\gamma^k & -k\gamma^{k} \\
        2k\gamma^{k} & -k\gamma^{k}
    \end{bmatrix}}_F
    \le
    8k\gamma^k=8k\rho(\Tb_{t,j})^k.
\end{align*}
Therefore, combining the two cases, we obtain the conclusion.
\end{proof}

\begin{lemma}[Bounding $\Norm{\prod_{i=1}^k(\Tb_{t,j}+\Delta_i)}_F$ with matrix power]\label{lem:2}
    For momentum matrices $\Tb_{t,j}+\Delta_i$ and $\Tb_{t,j}+\Delta$ where $\Tb_{t,j}$ $\Delta_i$, $\Delta$ claimed as 
    \begin{align*}
        \Tb = \begin{bmatrix}
            1+\beta-\eta_t\lambda_j & -\beta \\ 1 & 0
        \end{bmatrix}, \qquad
        \Delta = \begin{bmatrix}
            \delta_i &0 \\ 0 & 0
        \end{bmatrix}, \qquad
        \Delta = \begin{bmatrix}
            \delta &0 \\ 0 & 0
        \end{bmatrix},
    \end{align*}
    where $\delta_i>0$ and $\delta = \max_i\delta_i$. If 
    $
        (1+\beta-\eta_t\lambda_j)^2-4\beta\geq0,
    $
    it holds that
    \begin{align*}
        \Norm{\prod_{i=1}^k(\Tb_{t,j}+\Delta_i)}_F\le
        \Norm{\left(\Tb_{t,j}+\Delta \right)^k}_F.
    \end{align*}
\end{lemma}
\begin{proof}
First we consider the case that the eigenvalues of $\Tb_{t,j}$ $\gamma_1, \gamma_2\in \mathbb{R}$, which is equivalent to $(1+\beta-\eta_t\lambda_j)^2-4\beta\geq0$. Recall that in this case, the power of momentum matrix $\Tb_{t,j}$ is
\begin{align*}
    \Tb_{t,j}^k
    &=\left[\begin{matrix}\frac{\gamma_1^{k+1}-\gamma_2^{k+1}}{\gamma_1-\gamma_2}&\frac{-\beta(\gamma_1^{k}-\gamma_2^{k})}{\gamma_1-\gamma_2}\\\frac{\gamma_1^k-\gamma_2^k}{\gamma_1-\gamma_2}&\frac{-\beta(\gamma_2^{k-1}-\gamma_1^{k-1})}{\gamma_1-\gamma_2}\end{matrix}\right]\\
    &=\left[\begin{matrix} \sum_{j=0}^k\gamma_1^{j}\gamma_2^{k-1-j} & -\beta\sum_{j=0}^{k-1}\gamma_1^{j}\gamma_2^{k-2-j} \\ \sum_{j=0}^{k-1}\gamma_1^{j}\gamma_2^{k-2-j} & -\beta\sum_{j=0}^{k-2}\gamma_1^{j}\gamma_2^{k-3-j}\end{matrix}\right],
\end{align*}
where the second equality also holds for the case that $\gamma_1=\gamma_2$ and thus the lemma also holds for the case that $\gamma_1=\gamma_2$. We first consider the combination product form of ${\prod_{i=1}^{k}(\Tb_{t,j}+\Delta_i)}$ that
\begin{align*}
    &\prod_{i=1}^k(\Tb_{t,j}+\Delta_i)=\sum_{l_1+...+l_t+k_1+...+k_{t+1}=k}\Tb_{t,j}^{k_1}\Delta_{11}...\Delta_{1l_1}\Tb_{t,j}^{k_2}\Delta_{21}...\Delta_{2l_2}\Tb_{t,j}^{k_3}...\Delta_{t1}...\Delta_{tl_t}\Tb_{t,j}^{k_{t+1}}.
\end{align*}
The combination form of the two are of the same structure with different $\Delta_i$. If we consider one arbitrary combination term that
\begin{align*}
    \Sb=\Tb_{t,j}^{k_1}\Delta_{11}...\Delta_{1l_1}\Tb_{t,j}^{k_2}\Delta_{21}...\Delta_{2l_2}\Tb_{t,j}^{k_3}...\Delta_{t1}...\Delta_{tl_t}\Tb_{t,j}^{k_{t+1}},
\end{align*}
we first proof by induction that $\Sb$ has the following property: 
\begin{enumerate}
    \item the first column of $\Sb$ is nonnegative and the second column of $\Sb$ is nonpositive;
    \item the absolute value of each entry of $\Sb$ monotonically increasing with respect to $\delta_{1},...,\delta_{k}$.
\end{enumerate}
We call $\Tb_{t,j}^{k_i}$ or $\Delta_{ij}$ one multiple component of $\Sb$ in the following proof. And we denote $\Sb_p$ the product of the first $p$ multiple component of $\Sb$ in the following proof. The first multiple component of $\Sb$ can be $\Sb_1=\Tb_{t,j}^{k_1}$ or $\Sb_1=\Delta_{11}$, which satisfies the two desired properties naturally. Then we assume that the product of the first $p$ multiple component $\Sb_p$ satisfies the two properties. We discuss $\Sb_{p+1}$ in cases that
\begin{enumerate}
    \item if the $p$-th multiple component is $\Tb_{t,j}^{i}$, where $i$ represents an arbitrary integer, then the $(p+1)$-th multiple component should be $\Delta_{i'}$, where $i'$ also represents an arbitrary integer, or the $p$-th and $(p+1)$-th component can be merged. Then it holds that
    \begin{align*}
        \Sb_{p+1}=\Sb_p\Delta_{i'}=\left[\begin{matrix}
            \Sb_{p,11} & \Sb_{p,12} \\ \Sb_{p,21} & \Sb_{p,22}
        \end{matrix}\right]
        \left[\begin{matrix}
            \delta_{i'} & 0 \\ 0 & 0
        \end{matrix}\right]
        =
        \left[\begin{matrix}
            \delta_{i'}\Sb_{p,11} & 0 \\ \delta_{i'}\Sb_{p,21} & 0
        \end{matrix}\right].
    \end{align*}
    Thus if the two properties hold for $p$, it also holds for $p+1$ in this case.
    \item if the $p$-th multiple component is $\Delta_{i}$, where $i$ represents an arbitrary integer, and the $(p+1)$-th multiple component is $\Delta_{i+1}$, then it holds that
    \begin{align*}
        \Sb_{p+1}=\Sb_p\Delta_{i+1}=\left[\begin{matrix}
            \Sb_{p,11} & \Sb_{p,12} \\ \Sb_{p,21} & \Sb_{p,22}
        \end{matrix}\right]
        \left[\begin{matrix}
            \delta_{i+1} & 0 \\ 0 & 0
        \end{matrix}\right]
        =
        \left[\begin{matrix}
            \delta_{i+1}\Sb_{p,11} & 0 \\ \delta_{i+1}\Sb_{p,21} & 0
        \end{matrix}\right].
    \end{align*}
    Thus if the two properties hold for $p$, it also holds for $p+1$ in this case.
    \item if the $p$-th multiple component is $\Delta_{i}$, where $i$ represents an arbitrary integer, and the $(p+1)$-th multiple component is $\Tb_{t,j}^{i'}$, then it holds that
    \begin{align*}
        \Sb_{p}=\Sb_{p-1}\Delta_{i}=\left[\begin{matrix}
            \Sb_{p-1,11} & \Sb_{p-1,12} \\ \Sb_{p-1,21} & \Sb_{p-1,22}
        \end{matrix}\right]
        \left[\begin{matrix}
            \delta_{i} & 0 \\ 0 & 0
        \end{matrix}\right]
        =
        \left[\begin{matrix}
            \delta_{i}\Sb_{p-1,11} & 0 \\ \delta_{i}\Sb_{p-1,21} & 0
        \end{matrix}\right],
    \end{align*}
    which implies that $\Sb_{p,12}=\Sb_{p,22}=0$, thus we can substitute that
    \begin{align*}
        \Sb_{p+1}=\Sb_p\Tb_{t,j}^{i'}=\left[\begin{matrix}
            \Sb_{p,11} & 0 \\ \Sb_{p,21} & 0
        \end{matrix}\right]
        \left[\begin{matrix}
            t_{11} & t_{12} \\ t_{21} & t_{22}
        \end{matrix}\right]
        =
        \left[\begin{matrix}
            \Sb_{p,11}t_{11} & \Sb_{p,11}t_{12} \\ \Sb_{p,21}t_{11} & \Sb_{p,21}t_{12}
        \end{matrix}\right].
    \end{align*}
    As $t_{11},\Sb_{p,11},\Sb_{p,21}$ are nonnegative, $t_{12}$ is nonpositive, the two properties also hold for $\Sb_{p+1}$.
\end{enumerate}

Therefore, by induction we proof that the two properties hold for any combination term $\Sb$. And it is easy to verify that the properties also hold for their summation $\prod_{i=1}^k(\Tb+\Delta_i)$. And because the definition of frobenius norm, when the two properties hold, $\Norm{\prod_{i=1}^k(\Tb+\Delta_i)}_F$ is monotonically increasing with respect to $\delta_1,...\delta_k$ as well. Therefore, it holds that
\begin{align*}
    \Norm{\prod_{i=1}^k(\Tb_{t,j}+\Delta_i)}_F \le \Norm{\prod_{i=1}^k(\Tb_{t,j}+\Delta)}_F
    = \Norm{(\Tb_{t,j}+\Delta)^k}_F.
\end{align*}
\end{proof}

\begin{lemma}[$\rho$ bound by $\eta,\lambda,\beta$ in real eigenvalue case]\label{lem:rho_eta_beta}
    For momentum matrix
    \begin{align*}
        \Tb=\left[\begin{matrix}
            1+\beta-\eta\lambda & -\beta \\ 1 & 0
        \end{matrix}\right],
    \end{align*}
    if the discriminant $(1+\beta-\eta\lambda)^2-4\beta>0$
    the spectral radius of $\Tb$ is
    \begin{align*}
        \rho(\Tb)=\frac{1+\beta-\eta\lambda+\sqrt{(1+\beta-\eta\lambda)^2-4\beta}}{2}.
    \end{align*}
    And it holds that
    \begin{align*}
        \rho(\Tb) \leq 1-\frac{\eta\lambda}{2}-\frac{\eta\lambda}{4\left(1-\sqrt{\beta}\right)}.
    \end{align*}
\end{lemma}
\begin{proof}
It holds that
\begin{equation*}
\begin{aligned}
    \rho(\Tb)&=\frac{1}{2}\left[1+\beta-\eta\lambda+\sqrt{(1+\beta-\eta\lambda)^2-4\beta}\right] \\
    &= 
    \frac{1}{2}\left[1+\beta-\eta\lambda+\sqrt{\left(1-\sqrt{\beta}\right)^2-\eta\lambda}\cdot\sqrt{\left(1+\sqrt{\beta}\right)^2-\eta\lambda}\right] \\
    &\le
    \frac{1}{2}\left[1+\beta-\eta\lambda+\left(1+\sqrt{\beta}\right)\sqrt{\left(1-\sqrt{\beta}\right)^2-\eta\lambda}\right] \\
    &=
    \frac{1}{2}\left[1+\beta-\eta\lambda+\left(1-\beta\right)\sqrt{1-\frac{\eta\lambda}{\left(1-\sqrt{\beta}\right)^2}}\right] \\
    &\le
    \frac{1}{2}\left[1+\beta-\eta\lambda+\left(1-\beta\right)\left(1-\frac{\eta\lambda}{2\left(1-\sqrt{\beta}\right)^2}\right)\right] \\
    &=
     \frac{1}{2}\left[2-\eta\lambda-\frac{(1-\beta)\eta\lambda}{2(1-\sqrt{\beta})^2}\right] 
    \le
    \frac{1}{2}\left[2-\eta\lambda-\frac{\eta\lambda}{2(1-\sqrt{\beta})}\right] \\
    &=
    1-\frac{\eta\lambda}{2}-\frac{\eta\lambda}{4\left(1-\sqrt{\beta}\right)},
\end{aligned}
\end{equation*}
where the second last inequality holds because of the fact that $\sqrt{1-x} \le 1-x/2$ for all $x\in(0,1]$.
\end{proof}

\begin{lemma}\label{thm:main}
For $\beta\in [0,1)$, $\Tb_{t,j}$ defined as
\begin{align*}
    \Tb_{t,j}=\left[\begin{matrix}
            1+\beta-\eta_t\lambda_j & -\beta \\ 1 & 0
        \end{matrix}\right],
\end{align*}
 


    if the discriminant of $\Tb_{t,j}$ satisfies that $(1+\beta-\eta_t\lambda_j)^2-4\beta\geq0$, it holds that
    \begin{align*}
        \Norm{\prod_{l=t+1}^{t+k}\Tb_{l,j}}\le& \min\left(32k, \frac{8}{\sqrt{\Abs{(1+\beta-\eta_{t+k}\lambda_j)^2-4\beta}}} \right)\rho(\Tb_{t+k,j})^{k}
        .
    \end{align*}
 
    
\end{lemma}
\begin{proof}
    Combining Lemma \ref{lem:1} and \ref{lem:2}, one can verify that
    \begin{align*}
        \Norm{\prod_{l=t+1}^{t+k}\Tb_{l,j}}\le& \Norm{\prod_{l=t+1}^{t+k}\Tb_{l,j}}_F 
        \overset{\ref{lem:2}}{\le}
        \Norm{\Tb_{t+k,j}^{k}}_F \\
        \overset{\ref{lem:1}}{\le}& \min\left(32k, \frac{8}{\sqrt{\Abs{(1+\beta-\eta_{t+k}\lambda_j)^2-4\beta}}} \right)\rho(\Tb_{t+k,j})^{k},
    \end{align*}
    which concludes the proof.
\end{proof}




\section{Application to Prove Momentum}
From bias-variance decomposition, we have that the total error can be expressed by the two following terms, which are bias and variance respectively:
\begin{align*}
    B&\overset{\triangle}{=} \sum_{j=1}^d \lambda_j\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{1,j}}^2\mathbb{E}\Norm{\left( \mathbf{\Pi}^\top\mathbf{V}^\top\left[\begin{matrix}
        w_1-w_* \\ w_0-w_*
    \end{matrix}\right] \right)_{2j-1:2j}}^2,\\
    V&\overset{\triangle}{=} \sigma^2 \sum_{j=1}^d \lambda_j^2 \sum_{\tau=1}^{T-1} \eta_{\tau}^2\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{\tau+1,j}}^2.
\end{align*}
Next we try to make use of Theorem \ref{thm:main} to prove bound for them.
\begin{theorem}[Main result for momentum]\label{thm:momentum}
    Given a quadratic objective $f(w)$ and a step decay learning rate scheduler with $k_l\equiv T/n_l$ that satisfies
    \begin{enumerate}
        \item the first stage stepsize
        \begin{align*}
            \eta_1' \approx \frac{1}{L}
        \end{align*}
        \item the stepsize decay
        \begin{align*}
            \eta_{l+1}'=\frac{\eta_l'}{C}
        \end{align*}
        \item the last stage stepsize
        \begin{align*}
            \eta_{n_l}' \leq \frac{3\eta_1'}{4\kappa}
        \end{align*}
        \item the stage length
        \begin{align*}
            \Theta(\sqrt{\kappa}\log \kappa)\leq k_l \leq \theta(\frac{T}{\log \kappa})
        \end{align*}
    \end{enumerate}
    If number of iterations $T\geq \Omega\left({\sqrt{\kappa}\left(\log \kappa\right)^2}\right)$, such scheduler exists, and with momentum set to
    \begin{align*}
        \beta = \left( 1 -  \sqrt{\eta_1\mu} \right)^2,
    \end{align*}
    the output of algorithm satisfies
    \begin{align*}
        &\mathbb{E}[f(w_{T})-f(w_*)] 
        \le
        \mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right]\cdot \Tilde{O}\left( \exp\left( -\frac{T}{\sqrt{\kappa}} \right) \right)
        +
        O\left(\frac{d\sigma^2}{T}f^2(T)\right).
    \end{align*}
    \textcolor{red}{The Constants haven't finished yet. It will be done maybe after the $f(T)$ and some other details are settled.}
\end{theorem}

\subsection{Settings and Notations}\label{sec:settings}
\textcolor{red}{Notice:} In the following proof, we assume that $T\geq\Tilde{\Omega}(\sqrt{\kappa})$.

Also we set a two phase $\beta$ with $\beta = \left(1-\sqrt{\eta_1\mu}\right)^2$, where $\eta_1=\Theta(1/L)$ for the first stage where $\eta_1=\Theta(1/L)$ and $\beta=\left(1-\frac{f}{T} \right)$ for the rest stages, where $f\equiv f(T,\kappa)$ is a pending function. As $T\geq\Tilde{\Omega}(\sqrt{\kappa})$, one can check that $\beta\geq\beta$. And for the popular case that $T=\Tilde{\Theta}(\sqrt{\kappa})$, the two phase $\beta$ is almost the same.

We use $\eta_t$ to denote the stepsize used in iteration $t$ and $\eta_l'$ to denote the stepsize used in stage $l$. We use $k_l$ to denote the length of stage $l$ and $n_l$ to denote the number of stages. We denote $C>1$ as the decay factor, which mean that $\eta_{l-1}'=C\eta_{l}'$. 

\subsection{Bounding Bias}
We first present a lemma to simplify our proof.
\begin{lemma}\label{lem:stage_less_1}
    Under the assumptions in Section \ref{sec:settings}, for all stage $l>1$ if
    \begin{align*}
        \eta_l'\lambda_j > (1-\sqrt{\beta})^2,
    \end{align*}
    and with requirements:
    \begin{enumerate}
        \item the length of the stage
        \begin{align*}
            k_l \geq \frac{T}{f}\cdot\log T^2
        \end{align*}
    \end{enumerate}
    it holds that
    \begin{align*}
        \Norm{\left(\Tb_{l,j}'\right)^{k_l}} \le 1.
    \end{align*}
\end{lemma}
\begin{proof}
    In this case, the eigenvalues of $\Tb_{l_{\text{start}}}$It holds that
    \begin{align*}
     \Norm{\left(\Tb_{l,j}'\right)^{k_l}} \le& \Norm{\left(\Tb_{l,j}'\right)^{k_l}}_F 
        \overset{\ref{lem:1}}{\le}
        8k_l\rho(\left(\Tb_{l,j}'\right)^{k_l})^{k_l} = 8k_l(\sqrt{\beta})^{k_l} \\
        \leq&
        8k_l\left( 1-\frac{f}{T} \right)^{\frac{T}{f}\cdot\log T^2} \\
        \leq&
        1.
    \end{align*}
\end{proof}
Then referencing the original paper, we can bound bias as follow.
\begin{lemma}[Bounding bias]\label{lem:bias}
    Under the assumptions in Section \ref{sec:settings}, it holds that
    \begin{align*}
        B \leq \mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right]\cdot \Tilde{O}\left( \exp\left( -\frac{T}{\sqrt{\kappa}} \right) \right)
    \end{align*}
    with requirements:
    \begin{enumerate}
        \item for momentum factor
        \begin{align}\label{eq:req_bias_beta}
            \beta=(1-\sqrt{\eta_1'\mu})^2.
        \end{align}
        \item for stage length
        \begin{align}\label{eq:req_bias_k}
            k_1 \ge \Tilde{\Omega}\left(\frac{T}{f}\right)
        \end{align}
    \end{enumerate}
\end{lemma}
\begin{proof}
    From vairance-bias decomposition, we have
    \begin{equation}
    \begin{aligned}
        B&= \sum_{j=1}^d \lambda_j\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{1,j}}^2\mathbb{E}\Norm{\left( \mathbf{\Pi}^\top\mathbf{V}^\top\left[\begin{matrix}
        w_1-w_* \\ w_0-w_*
    \end{matrix}\right] \right)_{2j-1:2j}}^2\\
    &= \sum_{j=1}^d \lambda_j\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{1,j}}^2\mathbb{E}\Norm{\left( \mathbf{\Pi}^\top\mathbf{V}^\top\Tilde{\wb}_1 \right)_{2j-1:2j}}^2 \\
    &=
    \sum_{j=1}^d \lambda_j\Norm{\left(\Tb_{n_l,j}'\right)^{k_{n_l}}\left(\Tb_{n_{l-1},j}'\right)^{k_{n_{l-1}}}...\left(\Tb_{1,j}'\right)^{k_{1}}}^2 \mathbb{E}\Norm{\left( \mathbf{\Pi}^\top\mathbf{V}^\top\Tilde{\wb}_1 \right)_{2j-1:2j}}^2 \\
    &\overset{\ref{lem:stage_less_1}}{\le}
    \sum_{j=1}^d \lambda_j\Norm{\left(\Tb_{1,j}'\right)^{k_{1}}}^2 \left(\frac{8}{\sqrt{(1+\beta-\eta_{T-1}\lambda_j)^2-4\beta}}\right)^2 \mathbb{E}\Norm{\left( \mathbf{\Pi}^\top\mathbf{V}^\top\Tilde{\wb}_1 \right)_{2j-1:2j}}^2 \\
    &\le
    \frac{256T^2}{f^2}\Norm{\left(\Tb_{1,d}'\right)^{k_{1}}}^2\cdot\mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right] \\
    &\le
    \frac{256T^2}{f^2}\left(8k_1\rho\left(\Tb_{1,d}'\right)^{k_1} \right)^2\cdot\mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right] \\
    &\le
    \frac{256T^2}{f^2}\left(8k_1\left(\sqrt{\beta}\right)^{k_1} \right)^2\cdot\mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right] \\
    &=
    \frac{256T^2}{f^2}\left(8k_1\left(1-\sqrt{\eta_1'\mu}\right)^{k_1} \right)^2\cdot\mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right] \\
    &\leq
    \exp\left( 14\log2+2\log k_1+2\log \frac{T}{f}-2k_1\sqrt{\eta_1'\mu} \right)\cdot\mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right] \\
    &\approx \mathbb{E}\left[ f(w_0)+f(w_1)-2f(w_*) \right]\cdot \Tilde{O}\left( \exp\left( -\frac{T}{f\sqrt{\kappa}} \right) \right),
    \end{aligned}
    \end{equation}
where the second inequality comes from the original paper page 45-46 and here it remains the same. And the last inequality is because of the fact that $1-x\leq \exp(-x)$ for $x\geq0$.
\end{proof}

\subsection{Bounding Variance}

\begin{lemma}[Bounding variance]\label{lem:var}
    Under the assumptions in Section \ref{sec:settings}, it holds that
    \begin{align*}
        V  \leq \frac{f^2}{T}.
    \end{align*}
    with requirements:
    \begin{enumerate}
        \item for momentum factor
        \begin{align}\label{eq:req_var_beta}
            \beta=\left(1-\sqrt{\eta_1'\mu}\right)^2, \quad \beta = \left(1-\frac{f}{T}\right)^2.
        \end{align}
        \item the first stepsize $\eta_1$ or $\eta_1'$ (\textcolor{red}{comes from bounding variance of complex near boundary and far from boundary})
        \begin{align}\label{eq:req_var_eta_1}
            \eta_1'L \leq 1
        \end{align}
        \item the pending function $f$
        \begin{align}\label{eq:req_var_f}
            f \leq \frac{T}{2(C-1)}
        \end{align}
        \item the last stepsize $\eta_{T-1}$ or $\eta_{n_l}'$ (\textcolor{red}{comes from bounding variance in real-eigenvalue case}) 
        \begin{align}\label{eq:req_var_eta_T}
            \eta_{n_l}'\leq \min_j\left( \frac{3(1-\sqrt{\beta})^2}{4\lambda_j} \right) \Leftrightarrow \eta_{n_l}' \leq \frac{3\eta_1}{4\kappa}
        \end{align}
        It is equivalent to the requirement that
        \begin{align*}
            \left( \frac{1}{C}\right)^{n_l-1} = \frac{\eta_{T-1}}{\eta_1} \le \frac{3}{4\kappa} \Leftrightarrow n_l=\frac{T}{k_l} \geq \log \kappa.
        \end{align*}
        \item the stage length $k_l$ (\textcolor{red}{comes from bounding variance of complex near boundary})
        \begin{align}\label{eq:req_var_k_l}
            k_{l} \le \frac{T}{\log T} 
        \end{align}
        \item The total iteration number $T$
        \begin{align}\label{eq:req_var_T}
            k_l\log \kappa = \Theta\left(\sqrt{\kappa}\left(\log\kappa\right)^2\right)\geq T\geq k_l =\Theta\left( \sqrt{\kappa}\log \kappa \right)
        \end{align}
    \end{enumerate}
\end{lemma}

\begin{proof}
If we denote
\begin{align*}
    V_{t,j}&\overset{\triangle}{=} \eta_{t}^2\lambda_j^2 \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2,
\end{align*}
we desire for all $t,j$, $V_{t,j}$ can be bounded by
\begin{align*}
    V_{t,j} = \Tilde{O}\left(\frac{1}{T^2}\right).
\end{align*}
\textbf{Case Real-Eigenvalue with Small Stepsize}: We first consider the case that $\Tb_{t,j}$ only has real eigenvalues. This case is equivalent to that
\begin{align*}
    (1+\beta-\eta_{t}\lambda_j)^2- 4\beta \geq 0.
\end{align*}
It is also equivalent to that
\begin{align}\label{eq:var_eig_real}
    \eta_{t}\lambda_j \leq (1-\sqrt{\beta})^2=\eta_1'\mu.
\end{align}
And in this case we further assume that $\eta_t\lambda_j$ is small enough that
\begin{align*}
    \eta_t\lambda_j \le \frac{f}{T\sqrt{\kappa}},
\end{align*}
where $f\equiv f(T,\kappa)$ is a pending polynomial of $\log T$ and $\log \kappa$.   
From the fact that Frobenius norm of a matrix is always larger than $\ell_2$ norm and using Theorem \ref{thm:main} we can obtain that
\begin{align*}
    \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}} \le& \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}_F \\
    \overset{\ref{thm:main}}{\le}&
    \min\left(8(T-1-\tau), \frac{8}{\sqrt{{(1+\beta-\eta_{T-1}\lambda_j)^2-4\beta}}} \right)\rho(\Tb_{T-1,j})^{T-1-\tau} \\
    \le& 
    \frac{8}{\sqrt{{(1+\beta-\eta_{T-1}\lambda_j)^2-4\beta}}}\rho(\Tb_{T-1,j})^{T-1-\tau} \\
    =&
    \frac{8}{\sqrt{{(1+\beta-\eta_{n_l}'\lambda_j)^2-4\beta}}}\rho(\Tb_{T-1,j})^{T-1-\tau}
\end{align*}
Then we analyze the right hand side term by term. First it holds that
\begin{equation}\label{eq:var_product_real}
\begin{aligned}
    \sqrt{{(1+\beta-\eta_{n_l}'\lambda_j)^2-4\beta}} &=\sqrt{(1-\sqrt{\beta})^2-\eta_{n_l}'\lambda_j}\cdot\sqrt{(1+\sqrt{\beta})^2-\eta_{n_l}'\lambda_j} \\
    &\ge
    \sqrt{(1-\sqrt{\beta})^2-\eta_{n_l}'\lambda_j} \\
    &\overset{(\ref{eq:req_var_eta_T})}{\geq} \frac{1}{2}(1-\sqrt{\beta }) 
    \overset{(\ref{eq:req_var_beta})}{=} \frac{1}{2}\sqrt{\eta_1'\mu} 
\end{aligned}
\end{equation}
And from the properties of the matrices $\Tb$, $\rho(\Tb_{t,j})<1$ holds for all $t,j$. Combining all above we can obtain that for $t,j$ satisfying $\eta_t\lambda_j\leq f/\left(T\sqrt{\kappa}\right)$, it holds that

\begin{equation*}
\begin{aligned}
    V_{t,j}&=\eta_{t}^2\lambda_j^2 \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\le
    \left(\frac{f}{T\sqrt{\kappa}}\right)^2\left( \frac{8}{\sqrt{{(1+\beta-\eta_{n_l}'\lambda_j)^2-4\beta}}}\right)^2 \\
    &\le
    \frac{f^2}{T^2\kappa}\frac{64}{\left(\frac{1}{2}\sqrt{\eta_1'\mu}\right)^2} = \frac{256f^2}{T^2\kappa\eta_1'\mu}.
\end{aligned}
\end{equation*}
Moreover, if $t\in S_l$ is an iteration in the last stage that satisfies $\eta_t\lambda_j\geq f/(T\sqrt{\kappa})$, it holds that
\begin{align*}
    \eta_t\lambda_j \leq \frac{Cf}{T\sqrt{\kappa}}.
\end{align*}
Then we have 
\begin{align*}
    V_{t,j}&=\eta_{t}^2\lambda_j^2 \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\le
    \left(\frac{Cf}{T\sqrt{\kappa}}\right)^2\left( \frac{8}{\sqrt{{(1+\beta-\eta_{n_l}'\lambda_j)^2-4\beta}}}\right)^2 \\
    &\le
    \frac{C^2f^2}{T^2\kappa}\frac{64}{\left(\frac{1}{2}\sqrt{\eta_1'\mu}\right)^2} = \frac{256C^2f^2}{T^2\kappa\eta_1'\mu}.
\end{align*}

\textbf{Case Real-Eigenvalue with Large Stepsize}: Then we consider the case that$\Tb_{t,j}$ only has real eigenvalues. This case is equivalent to that
\begin{align*}
    (1+\beta-\eta_{t}\lambda_j)^2- 4\beta \geq 0.
\end{align*}
It is also equivalent to that
\begin{align}\label{eq:var_eig_real_2}
    \eta_{t}\lambda_j \leq (1-\sqrt{\beta})^2=\eta_1'\mu.
\end{align}
In this case we further assume that $\eta_t\lambda_j$ is large enough that
\begin{align*}
    \eta_t\lambda_j \ge \frac{Cf}{T\sqrt{\kappa}}
\end{align*}
as the case that $\eta_t\lambda_j\le Cf/(T\sqrt{\kappa})$ has been discussed in the first case. From the requirement that $T=\Tilde{\Omega}\left(\sqrt{\kappa}\right)$ we know that such stage exists. Then according to Lemma \ref{lem:rho_eta_beta}, it holds that
\begin{align*}
    \rho(\Tb_{t,j})&=\frac{1}{2}\left[1+\beta-\eta_t\lambda_j+\sqrt{(1+\beta-\eta_t\lambda_j)^2-4\beta} \right] \\
    &\overset{\ref{lem:rho_eta_beta}}{\le}
    1-\frac{\eta_t\lambda_j}{4\left(1-\sqrt{\beta}\right)} = 1 - \frac{\eta_t\lambda_j}{4\sqrt{\eta_1\mu}} \\
    &\approx
    1 - \frac{Cf}{4T}.
\end{align*}
Thus if we denote $t_*$ to be the first iteration that $\eta_{t_*}\lambda_j\leq f/\left(T\sqrt{\kappa}\right)$, it holds that
\begin{equation*}
\begin{aligned}
    V_{t,j}&=\eta_{t}^2\lambda_j^2 \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\le
    \eta_{t}^2\lambda_j^2\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t_*,j}}^2\Norm{\Tb_{t_*-1,j}\Tb_{t_*-2,j}...\Tb_{t+1,j}}^2 \\
    &\le
   \eta_{t}^2\lambda_j^2\left(\frac{8}{\sqrt{{(1+\beta-\eta_{n_l}'\lambda_j)^2-4\beta}}}\right)^2\left( 1-\frac{Cf}{4T}\right)^{2(t_*-t-1)} \\
    &\le
    \eta_{t}^2\lambda_j^2\frac{64}{\left(\frac{1}{2}\sqrt{\eta_1'\mu}\right)^2}\left( 1-\frac{Cf}{4T}\right)^{2(t_*-t-1)} 
    \le
    \eta_{t}^2\lambda_j^2\frac{64}{\left(\frac{1}{2}\sqrt{\eta_1'\mu}\right)^2}\left( 1-\frac{Cf}{4T}\right)^{2k_l} \\
    &\le
    \frac{256C^2f^2\eta_1'\mu}{T^2}.
\end{aligned}
\end{equation*}

\textbf{Case Complex Small Stepsize:} Then we consider the case that $\Tb_{t,j}$ has complex eigenvalues which is equivalent to that
\begin{equation}\label{eq:var_eig_complex}
\begin{aligned}
    \eta_t\lambda_j > (1-\sqrt{\beta})^2 &= \eta_1\mu
\end{aligned}
\end{equation}
and also $\Tb_{t,j}$ is near the boundary, which we define as the stepsize of the next stage, denoted by $\eta_{l+1}'$, satisfies Equation (\ref{eq:var_eig_real}), which means that the corresponding momentum matrix has only real eigenvalues. Thus if we denote $t_*$ to be the first iteration in the $l+1$ stage, consider the spectral raidus of the $l+1$ stage, it holds that
\begin{equation}
\begin{aligned}
    \rho(\Tb_{t_*,j})=&\frac{1}{2}\left[ 1+\beta-\eta_{l+1}'\lambda_j + \sqrt{(1+\beta-\eta_{l+1}'\lambda_j)^2-4\beta} \right] \\
    \overset{\ref{lem:rho_eta_beta}}{\le}&
    1-\frac{\eta_{l+1}'\lambda_j}{4(1-\sqrt{\beta})} = 1 - \frac{\eta_{l+1}'\lambda_j}{4\sqrt{\eta_1'\mu}} \\
    \le&
    1 - \frac{\eta_1'\mu}{4C\sqrt{\eta_1'\mu}} = 1 - \frac{\sqrt{\eta_1'\mu}}{4C}
\end{aligned}
\end{equation}
thus we have
\begin{align*}
    \rho(\Tb_{t_*,j})^{k_{l+1}} \le& (1-\frac{f}{2CT})^{k_{l+1}} \\
    \overset{(\ref{eq:req_var_k_l})}{\le}&
    (1-\frac{f}{2CT})^{\frac{2CT}{f}\log T} \\
    \le&
    e^{-\log T}=\frac{1}{T^4}
\end{align*}

and substituting we have

\begin{equation}\label{eq:var_complex_near_mid_prod}
\begin{aligned}
    \Norm{\Tb_{t_*+k_{l+1}-1,j}\Tb_{t_*+k_{l+1}-2,j}...\Tb_{t_*,j}} &= \Norm{\left(\Tb_{l+1}'\right)^{k_{l+1}}} \le \Norm{\left(\Tb_{l+1}'\right)^{k_{l+1}}}_F \\
    &\overset{\ref{lem:1}}{\le}
    8k_{l+1} \rho(\Tb_{t_*,j})^{k_{l+1}} \\
    &\overset{(\ref{eq:req_var_k_l})}{\le}
    8T\cdot \frac{1}{T^4} = \frac{8}{T^3}.
\end{aligned}
\end{equation}

Thus we have
\begin{equation}
\begin{aligned}
    V_{t,j}&=\eta_{t}^2\lambda_j^2 \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\le
    (C\eta_{l+1}'\lambda_j)^2\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\overset{(\ref{eq:var_eig_real})}{\le}
    \frac{C^2f^4}{T^4}\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\le
    \frac{C^2f^4}{T^4}\Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t_*+k_{l+1},j}}^2 \Norm{\Tb_{t_*+k_{l+1}-1,j}\Tb_{T-2,j}...\Tb_{t_*,j}}^2 \Norm{\Tb_{t_*-1,j}\Tb_{t_*-2,j}...\Tb_{t+1,j}}^2 \\
    &\overset{(\ref{eq:var_product_real})}{\le}
    \frac{C^2f^4}{T^4}\cdot \frac{256T^2}{f^2} \Norm{\Tb_{t_*+k_{l+1}-1,j}\Tb_{T-2,j}...\Tb_{t_*,j}}^2 \Norm{\Tb_{t_*-1,j}\Tb_{t_*-2,j}...\Tb_{t+1,j}}^2 \\
    &\overset{(\ref{eq:var_complex_near_mid_prod})}{\le}
    \frac{256C^2f^2}{T^2}\cdot\frac{8}{T^3}\Norm{\Tb_{t_*-1,j}\Tb_{t_*-2,j}...\Tb_{t+1,j}}^2 \\
    &\overset{\ref{lem:1}}{\le}
    \frac{2^{11}C^2f^2}{T^5}\cdot (8k_l)^2 \le \frac{2^{17}C^2k_l^2f^2}{T^5} \\
    &\overset{ }{\le}
    \frac{2^{17}C^2f^2}{T^3} 
\end{aligned}
\end{equation}

\textbf{Case Complex Large Stepsize:} Finally we consider the case that $\Tb_{t,j}$ has complex eigenvalues which is equivalent to Equation (\ref{eq:var_eig_complex}) and also $\Tb_{t,j}$ is far away from the boundary, which we define as the stepsize of the next stage can still satisfies Equation (\ref{eq:var_eig_complex}). Thus we consider that
\begin{equation}
    \begin{aligned}
    V_{t,j}&=\eta_{t}^2\lambda_j^2 \Norm{\Tb_{T-1,j}\Tb_{T-2,j}...\Tb_{t+1,j}}^2 \\
    &\overset{(\ref{eq:req_var_eta_1})}{\le}
    \Norm{\Tb_{T-1,j}...\Tb_{t_*,j}}^2\Norm{\left(\Tb_{l_*,j}'\right)^{k_{l_*}}}^2\Norm{\left(\Tb_{l_*-1,j}'\right)^{k_{l_*-1}}}^2...\Norm{\left( \Tb_{l_{t+1},j}'\right)^{l_{t+1}}}^2\Norm{\left( \Tb_{l_{t},j}'\right)^{l_{t}-t}}^2 \\
    &\overset{(\ref{eq:var_product_real})}{\le}
    \frac{256T^2}{f^2}\Norm{\left(\Tb_{l_*,j}'\right)^{k_{l_*}}}^2\Norm{\left(\Tb_{l_*-1,j}'\right)^{k_{l_*-1}}}^2...\Norm{\left( \Tb_{l_{t+1},j}'\right)^{l_{t+1}}}^2\Norm{\left( \Tb_{l_{t},j}'\right)^{l_{t}-t}}^2 \\
    &\overset{\ref{lem:stage_less_1}}{\le}
    \frac{256T^2}{f^2}\Norm{\left(\Tb_{l_*,j}'\right)^{k_{l_*}}}^2\Norm{\left( \Tb_{l_{t},j}'\right)^{l_{t}-t}}^2 \\
    &\overset{\ref{lem:1}}{\le}
    \frac{256T^2}{f^2}\left( 8k_{l_*}\left(\sqrt{\beta}\right)^{k_{l_*}} \right)^2 \left( 8k_{l_t} \right)^2 
    \overset{(\ref{eq:req_var_beta})}{\le}
    \frac{2^{20}k_l^4T^2}{f^2}\left(1-\frac{f}{T}\right)^{2k_l} \\
    &\le
    \frac{2^{20}k_l^4T^2}{f^2}\left(1-\frac{f}{T}\right)^{2C\frac{T}{f}\log T^4} \leq \frac{2^{20}}{T^2} 
    \end{aligned}
\end{equation}

Therefore, combining the three cases, we have the result
\begin{align*}
    V = \sigma^2\sum_{j=1}^{d}\sum_{t=0}^{T-1}V_{t,j} \le& \sigma^2\sum_{j=1}^{d}\sum_{t=0}^{T-1} \frac{f^2}{T^2}   \overset{ }{\le} \frac{d\sigma^2}{T}f^2,
\end{align*}
which concludes the proof.

\end{proof}

\subsection{Proof of Theorem \ref{thm:momentum}}
Combining the above two sections and merging the requirements, we can verify that the theorem holds.

